Are current long-term video understanding datasets long-term?

Many real-world applications, from sport analysis to surveillance, benefit from automatic long-term action recognition. In the current deep learning paradigm for automatic action recognition, it is imperative that models are trained and tested on datasets and tasks that evaluate if such models actually learn and reason over long-term information. In this work, we propose a method to evaluate how suitable a video dataset is to evaluate models for long-term action recognition. To this end, we define a long-term action as excluding all the videos that can be correctly recognized using solely short-term information. We test this definition on existing long-term classification tasks on three popular real-world datasets, namely Breakfast, CrossTask and LVU, to determine if these datasets are truly evaluating long-term recognition. Our study reveals that these datasets can be effectively solved using shortcuts based on short-term information. Following this finding, we encourage long-term action recognition researchers to make use of datasets that need long-term information to be solved.

==> introduction.tex <==
\label{sec:introduction}

Many interesting actions happening in the real world are long-term. That is, they are composed of several short sub-actions, that we refer to as \textit{short-term actions}. %, that occur together over time to realize the long-term action. 
For an action to be \emph{long-term}, we deem that recognizing a single short term action is not enough, and  reasoning about the order and the relationshiop of short-term actions is required. 
Two examples of long-term actions, shown in Figure \ref{fig:fig1}, are \textit{winning a soccer game} and \textit{shoplifting in the supermarket}. To understand which team is winning a soccer game, it is necessary to recognize and count the goals scored since the beginning of the game. This requires observing short-term actions as %\textit{pass} the ball, 
\klamer{run and kick seems not esssential elements to winning; this is I think scoring a goal, which consists of having the ball enter the goal (not necessarily touching the net) while not off-side or another foul.} \textit{run}, \textit{kick} and \textit{ball entering the goal net} over time. Keeping track of sub-actions order is crucial: the short-term moment in which the ball enters the goal net is by itself not sufficient to recognize a win. For the other example, recognizing if a person is shoplifting, it is necessary to observe a person storing a product in their pocket \textit{and} leaving the supermarket without paying. In both examples, it is not possible to recognize the actions without reasoning multiple ordered short-term actions. 


% Many interesting actions happening in the real world are long-term. These type of actions are composed of several short sub-actions (henceforth \textit{short-term actions}) that occur together over time. To recognize long-term actions, it is necessary to recognize the short-term actions and reason about their order and relationship to one another. An example of long-term action is \textit{scoring a goal} in a soccer game (see Figure \ref{fig:fig1}). A goal is composed of short-term actions as \textit{kick} or \textit{pass} the ball, \textit{run}, and the \textit{ball entering the goal net}. A key characteristic of long-term actions is that a short-term action alone, e.g. the moment in which the ball enters the goal net, is by itself not sufficient to recognize the long-term action. In fact, the antecedent short-term actions, including the position of the strikers \textit{before} the ball is kicked, are necessary to differentiate a goal from an offside. \todo{Better example? supermarket; enough packing for a week?} 


\begin{figure*}[!ht]
\centering
\includegraphics[width=1\textwidth]{figures/Figure 1.pdf}
\caption{Example of truly long-term actions. \textit{Top:} Who is winning this soccer game? \klamer{it could be nice to include a "pass the ball" shot near the goal where it is clearly off-side}\textsuperscript{1}, \textit{Bottom:} Is this person shoplifting in the supermarket?\textsuperscript{2}. In both cases, it is not possible to answer correctly without considering multiple sub-actions together, their order and relations over time. To understand who is winning the soccer game, it is necessary to recognize and count the goals scored since the beginning of the game. %Recognizing a goal also requires temporal reasoning: the position of the attackers \textit{before} the ball kick, are necessary to differentiate a goal from an offside.
To recognize shoplifting, it is not enough to see a person putting a product in their pocket: also the sub-action \textit{leaving without paying} needs to occur. \\
  \small\textsuperscript{1} Source: \href{https://www.youtube.com/watch?v=p5laVw4EpYI}{YouTube};
  \small\textsuperscript{2} Source: \href{https://www.youtube.com/watch?v=5tVz7IChlWI}{YouTube} from movie \textit{Un povero ricco}, by Pasquale Festa Campanile (1983).
  \todo{remove soccer or just mention "counting the goals"}}
\label{fig:fig1}
\end{figure*}

Achieving automatic long-term action recognition is important because it can be used to solve real world problems, from analyzing sports videos, to understanding movies and recognizing threats in surveillance footage. 
% To make it possible, it is necessary to have a clear definition of long-term action that we can use to build long-term action recognition models and collect representative video datasets to train the models. 
% However, the definition of long-term action (also called long-range, long-form or complex) is vague in the literature. In this paper, we provide a definition for long-term action and investigate whether commonly used video datasets for long-term action recognition fall within this definition.
To make it possible, we need purpose-built computer vision models and representative long-term action datasets to train the models. 
%\klamer{I would put this part on CATER to the related work section, it does not add here to the story in the introduction} To diagnose whether models are capable to learn long-term information, Girdhar \textit{et al.} introduced the CATER dataset \cite{girdhar2019cater}, a synthetic dataset of moving shapes that can be localized correctly only by reasoning over their trajectories over time. Models that are not truly long-term fail on this dataset. 
%
Without representative training data, deep learning models are known to use shortcuts to solve classification tasks \cite{geirhos2020shortcut}.
In case of non-representative long-term action recognition datasets, a model could potentially learn to exploit short-term information, without encoding any long-term relations.
%
For example, if a model typically %%only sees 
videos with one goal and no offsides at training time, it might pick up the sub-action \textit{ball entering the goal net} and use it as a proxy to infer who is winning the game, ignoring the rest of the video. \klamer{Now you pose it as an overtraining case; I think that the actual point in this paper is not about overtraining, but rather on the unability of a model to actually model the long term relations, i.e. that it is not able to decide that a goal resulting from an off-side situation shall not be counted as a valid goal} This is dangerous because it can hurt the models performance on new videos with more goals and offsides. 

%\klamer{I propose we add a paragraph here which states the risk that long term action recognition models apply shortcuts. This should include a description on how that might happen, i.e. describe the common architecture and how such an architecture can learn a shortcut, as well as explain why such shortcuts would hinder true long term action recognition.}

\begin{figure}[ht!]
\centering
\includegraphics[width=0.5\textwidth]{figures/Breakfast_CrossTask_subaction_unicity.pdf}
\caption{We analyze two popular long-term datasets %the occurrences of short-term actions 
and count in how many long-term actions the short-term action appears.
A large percentage of short-term actions, 70.8\% for Breakfast (Coarse subactions) \cite{kuehne2014language} and 89.5\% for CrossTask \cite{zhukov2019cross}, only appear in one long-term action class. This means that often long-term actions can be recognized by recognizing a single short-term action. \todo{rephrase}
}
\label{fig:unique_subactions}
\end{figure}


In this work we aim to diagnose whether the \textit{actions} in real-world video datasets hold long-term properties. To this end, we formalize two requirements for an action to be long-term: 
(1) The action is \textit{recognizable only from multiple short-term actions} and not from a single short-term action. 
(2) The action maps to a \textit{single label}. 
The first requirement makes %\klamer{delete automatic} automatic 
long-term action recognition impossible without 
%\klamer{I suggest here to remove the capability of encoding information -- key here is IMHO the reasoning} the capability of encoding information and 
reasoning %\klamer{we shall define what we use here -- I thing we want to exclude global average pooling and global max pooling} 
over an extended time span. Consequently, models that cannot encode temporal order and long-term dependencies, for example based on \klamer{what do you mean here -- is pooling able to reason over an extended time span or not? Current text is not exclusive. You might want to something like 'excluding straightforward pooling operations' to make clear what you intend}pooling operations over the time dimension \cite{wang2016temporal}, cannot recognize long-term actions. 
%
\klamer{I do not get what you mean with 'Additionally' here} Additionally, long-term action recognition models cannot learn to exploit short-term shortcuts to recognize long-term actions. 
% \klamer{Suggest to rephrase to: The second requirements lead to discarding ... as long term action datasets} 
% We use the second requirement to discard 
The second requirement leads to discarding multi-label action recognition datasets, like Charades \cite{sigurdsson2016hollywood}, MultiTHUMOS \cite{yeung2018every} and EPIC-Kitchens \cite{damen2018scaling}, as long-term action datasets. In these datasets, the task is to recognize each short-term action contained in the videos. This task could be solved by a perfect short-term action recognition model, without the need of encoding long-term relations.

% Without this property, long-term action recognition models could learn to use short-term action recognition as a shortcut to recognize long-term actions. This is dangerous because it can hurt the models performance on new videos. 

% We define a \textit{long-term action} as a bag of short-term actions that maps to a single label. The characteristic property of long-term actions is that they are recognizable only by reasoning over multiple short-term actions, instead of considering only a single individual short-term action. 
% This property makes automatic long-term action recognition impossible without the capability of encoding information and reason over an extended time span. 
% Without this property, long-term action recognition models could learn to use short-term action recognition as a shortcut to recognize long-term actions. This is dangerous because it can hurt the models performance on new videos. 

% The characteristic property of long-term actions has consequences on the long-term action datasets, which should not contain videos recognizable by a single short-term action.

% For example, a dataset for goal recognition can only be a representative long-term action dataset if it contains instances of offsides. If not, a deep learning model trained without offside examples could erroneously learn to identify the long-term action \textit{scoring a goal} only from the short-term action \textit{ball entering the goal net}, thus performing poorly on new soccer videos containing offsides. 

Following the definition of our requirements, we introduce a method based on user studies to assess whether a video dataset contains %\klamer{how does our method address the representative aspect? - otherwise delete the word representative here} representative 
long-term action videos. In particular, we design two surveys \todo{Discuss comment below}
%\klamer{What I miss in the paper is a discussion WHY we resort to user studies. Before we already did the analysis that a perfect sub-action detector on Breakfast would work -- is that published work we can reference? Also we found that it is hard to train such a perfect sub action detector (unpublished work? ) which made us resort to user studies. Something along these lines should be (somewhere) in the paper.}\todo{Unfortunately we don't have any published work that we can cite. I understand that the explanation of what led to this work is missing. However, I don't know how to insert that story here without any papers to cite...} 
where users have to watch a video and predict the long-term action being performed in the video. In the \textit{Full Videos Survey}, the users can watch the full video, while in the \textit{Video Segments Survey} a separate group of users can watch only a single short clip 
%short-term action 
extracted from the full video. 
We measure the average action recognition accuracy of the users per video for each survey. % and for each of the considered datasets. 
%
The \textit{Full Videos Survey} gives an upper bound to the user long-term action recognition performance. Comparing the accuracy obtained from the \textit{Video Segments Survey} to the upper bound gives an estimate of how many videos in the dataset require long-term information to be correctly recognized. If the action recognition performance of the two groups of users is close, we can conclude that most of the videos in the dataset are not suitable to train models for long-term action recognition, because they can be recognized solely by exploiting short-term information.
%
% If the action recognition performance of the two groups of users is comparable, we can conclude that the videos are not truly long-term, because they can be recognized by looking at a single short-term action equally well as by looking at the full video.  \klamer{As the paragraph is currently written we should get the same results to make the claim a dataset is not long-term. Yet in the results there are not similar. Can we rephrase the wording here such that given the results (roughly similar) we still can make the claim these data sets are not truly long term -- or at least, would not be proper data sets to develop new long term action recognition models?}
%
%We \klamer{before we state we {\em introduce a method}, and that method consists of two studies. In that case, I would state here that we {\em apply our method} to the datasets, rather than to {\em include them in our study} -- this to stress the methodological aspect} include in our study 

We apply our proposed method to the popular Breakfast dataset \cite{kuehne2014language}, used in several works on long-term video understanding \cite{guo2022uncertainty, hussein2019timeception, li2022bridge, zhou2021graph}, and the instructional video dataset CrossTask \cite{zhukov2019cross}. Being composed of several steps that contribute to the completion of a task, instructional videos are suitable for our study on long-term actions. Finally, we include the Long-form Video Understanding benchmark (LVU) \cite{wu2021towards}, recently proposed for long-term video recognition tasks in movies. %\klamer{Can we make the claim that with this selection we have covered all current well-known long term video recognition datasets -- such a claim would really strengthen the paper}\todo{Probably not. Breakfast is used in almost every paper on the topic, but the other datasets are less popular. K=For LVU, I think that's because the dataset is recent and still not very well knows. Other datasets that are used a lot in the literature are the ones for multi-label classification, but we choose to exclude them.}
%
% We do not consider the popular Charades \cite{}, MultiTHUMOS \cite{} and EPIC-Kitchens \cite{damen2018scaling} datasets: being multi-label classification datasets, they already do not fall under our definition of long-term action datasets.
%
%
We implement the user studies on a Amazon Mechanical Turk \cite{mturk} and collect responses from more than 150 users. 
% Our results show that the Breakfast dataset can be recognized by looking at single short-term actions equally well as looking at the full videos. On the other hand, we find a statistically significant difference between the two surveys outcomes in Cross-Task and COIN.
% We conclude that Breakfast is not a representative long-term action recognition dataset because its actions can be recognized by looking at single, short video segments and ignoring the long-term information.  
Our results show that looking at a single short video segment is sufficient to recognize 90\% and 97.2\% of the analyzed videos from Breakfast and % the instructional video in 
CrossTask. Similarly, the relationships and scenes in the LVU dataset can be classified without long-term information. In the classification of the characters relationships and way of speaking, we find that many video segments are misclassified due to annotation noise.
%
% We conclude that Breakfast is not a representative long-term action recognition dataset because its actions can be recognized by looking at single, short video segments and ignoring the long-term information.  
We conclude that the aforementioned datasets %prediction \klamer{datasets not tasks?} tasks 
might not be suitable to %\klamer{not suitable to develop new methods for long term action recognition (learning long-term relations is not the goal we are after...) } learn long-term relations
develop new methods for long-term action recognition in videos, because they can be solved by ignoring the long-term information.
We recommend long-term video understanding researchers to be careful when using these datasets and encourage the community to collect more representative video datasets.
% opt for the Cross-Task and COIN datasets to investigate automatic long-term action recognition effectively.

In summary, the key contributions of our study can be outlined as follows:
%\begin{itemize}
(1) We provide a definition of long-term action dataset \klamer{datasets} 
that \klamer{should prevent} prevents long-term action recognition models to use traditional short-term action recognition as a shortcut to solve the task. 
(2) We introduce a method to investigate whether a video dataset \klamer{replace 'is representative to study the problem of automatic' by 'meets this definition of'} is representative to study the problem of automatic long-term action recognition.
%
% We use our method to analyze three current datasets used in long-term video understanding research. 
(3) We find that short-term information is, in most cases, sufficient to solve long-term video understanding tasks in three commonly used datasets. Thus, we recommend against using these datasets in further research on long term action recognition models. %actions in Breakfast, the instructional video classes in CrossTask, and the relationships and scenes in the LVU dataset.  
%\end{itemize}
%
% Upon paper acceptance, we will make our code and the responses gathered from the user studies publicly accessible.
Our code and the responses gathered from the user studies will be made available on our project page\footnote{TODO repo link}. 
